Adaptive Neighborhood Resizing for Stochastic Reachability in Multi-Agent Systems

We present DAMPC, a distributed, adaptive-horizon and adaptive-neighborhood algorithm for solving the stochastic reachability problem in multi-agent systems, in particular flocking modeled as a Markov decision process. At each time step, every agent calls a centralized, adaptive-horizon model-predictive control (AMPC) algorithm to obtain an optimal solution for its local neighborhood. Second, the agents derive the flock-wide optimal solution through a sequence of consensus rounds. Third, the neighborhood is adaptively resized using a flock-wide, cost-based Lyapunov function V. This way DAMPC improves efficiency without compromising convergence. We evaluate DAMPC's performance using statistical model checking. Our results demonstrate that, compared to AMPC, DAMPC achieves considerable speed-up (two-fold in some cases) with only a slightly lower rate of convergence. The smaller average neighborhood size and lookahead horizon demonstrate the benefits of the DAMPC approach for stochastic reachability problems involving any controllable multi-agent system that possesses a cost function.

==> algo_ampc.tex <==
%\SetAlgoSkip{}
\begin{algorithm}[ht!]
\small
	\SetKwFunction{particleswarm}{particleswarm}
    \SetKwFunction{Fitness}{cost}
    \SetKwFunction{RecedeHorizon}{RecedeHorizon}
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \DontPrintSemicolon
	\Input{$\M,\varphi,{h}_{\mathit{max}},m,B, \beta, \Fitness$}
	\Output{$\{\va^i\}_{1\leqslant i\leqslant\,m}$ \tcp*[l]{optimal control sequence}}
	\BlankLine
	Initialize $\ell_0\leftarrow J(s_0)$; $\widehat{J}\leftarrow\inf$;  $i\leftarrow 1$;  ${h}\leftarrow 1$; ${p}\leftarrow 2\beta h B$; $\Delta_0\leftarrow (\ell_0 - \varphi)/m$;
	\BlankLine
	\While{($\ell_{i-1} > \varphi)$ $\land$ $(i < m+h_\mathit{max})$}
	{
     	\tcp{find and apply first action of the best sequence of horizon $h$}
        $[\va^{h},\widehat{J}]\leftarrow$\particleswarm{$\Fitness,\M,p,h$};\\

        \eIf{$\ell_{i-1}-\widehat{J} > \Delta_i \lor h = h_{\mathit{max}}$} 
		{
        \tcp{if a new level or the maximum horizon is reached}
        	$\va^i\leftarrow \va^{h}_1$;
            $\M\leftarrow\M^{\va^i}$;
            \tcp*{apply the action and move to the next state}
			$\ell_i\leftarrow J(s(\M))$; \tcp*{update $\ell_i$ with the cost of the current state}
            $\Delta_i\leftarrow \min(\ell_i/(m-i),\ell_i)$; \tcp*{update the threshold on reaching the next level}
            $i \leftarrow i + 1$;
			${h} \leftarrow 1$;
			${p} \leftarrow 2\beta h B$; \tcp*{update parameters}
		}
		{
			${h} \leftarrow {h} + 1$;
            $p\leftarrow 2\beta h B$; \tcp*{increase the horizon}
		}
	}
	\caption{AMPC: Adaptive-Horizon MPC}
	\label{alg:ampc}
\end{algorithm}
\setlength{\floatsep}{1cm}



==> algo_avg_consensus.tex <==
%\SetAlgoSkip{}
\begin{algorithm}[ht!]
\small
	\SetKwFunction{localampc}{LocalAMPC}  
    \SetKwFunction{cost}{cost}
    \SetKwFunction{J}{J}
    \SetKwFunction{fixed}{Fixed}
    \SetKwFunction{fix}{Fix}
    \SetKwFunction{neigh}{Neighbors}
    \SetKwFunction{neighsize}{NeighSize}
    
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \SetKwFor{ParFor}{for}{do in parallel}{endfor} 
    \DontPrintSemicolon
	\Input{$\M\,{=}\,(S,A,T,J,I),\varphi,{h}_{\mathit{max}},m,B, \beta, \tau$}
	\Output{$\vs_0$, $\va^m\,{=}\,\{\va(t)\}_{1\leqslant t\leqslant\,m}$} 
	\BlankLine
	$\vs_0\leftarrow\mathrm{sample}(I)$; $\vs\leftarrow\vs_0$; 
    $\ell_0\leftarrow J(\vs)$; $\{\widehat{J}_i\}_{i\in{B}}\leftarrow\inf$;  $t\leftarrow 1$; $k\leftarrow B$; $\mathrm{checkpoint}\leftarrow 0$; \tcp*{Init}
	\BlankLine
	\While{($\ell_{t{-}1} > \varphi)$ $\land$ $(t < m)$}
	{
      \tcp{Birds run \localampc for their own neighborhoods}
      \ParFor{ $i=1:B$ } 
      {
      $N_i \leftarrow \neigh(i, k)$; \tcp{Find $k$ nearest neighbors of $i$}
      $\Delta_i \leftarrow J(\vs_{N_i})/(m{-}t)$;\\
  $({\vs}_{N_i},\va_{N_i}^{h_i},\widehat{J}_i)\leftarrow\localampc(\M,\vs_{N_i},{\va}_{N_i},\Delta_i,h_{max},\beta)$;
      }   
      \If (\tcp*[f]{Consensus rounds every $\tau$ time-steps}) {$t=\mathrm{checkpoint}+\tau$} 
      { 
      	\ForEach{$i=1:B$} 
        {
        	$\mathrm{NeighCount}\leftarrow 0$;
            $\overline{\va}_i\leftarrow \mathrm{first}(\va_{N_i}^{h_i})$;\\
            \ForEach{$j=1:B$ \tcp{Collect solution proposals from each neighborhood bird $i$ participated in}}
            {
            	\If{$i\in N_j$}
                {   	$\overline{\va}_i\leftarrow\overline{\va}_i+\va_{N_j}^{h_i}$;
                $\mathrm{NeighCount}\leftarrow\mathrm{NeighCount}+1$;
                }
            }
      	 $\overline{\va}_i\leftarrow\overline{\va}_i/\mathrm{NeighCount};$
        }
      	$\vs\leftarrow\overline{\vs}$;
      %$\vs\leftarrow\mathrm{sample}(T(\vs,\va(t)))$; 
      	\tcp*{Reconstruct the global state using new solutions}
      	\If {$\ell_{t{-}1} - J({\vs}) >\Delta$} {
        	$\ell_t\leftarrow J({\vs})$; \tcp*{Proceed to the next level}
      	}
      	$k \leftarrow \neighsize(J({\vs}), k)$; \tcp*{Adjust the neighborhood size}
		}
    }
    $t\leftarrow t{+}1$; $\mathrm{checkpoint}\leftarrow t$;
	\caption{Distributed Formation Control with Average Consensus}
	\label{alg:avg_consensus}
\end{algorithm}
\setlength{\floatsep}{1cm}



==> algo_fixed_order.tex <==
% \SetAlgoSkip{}
\begin{algorithm}[ht!]
\small
	 
    \SetKwFunction{cost}{cost}
    \SetKwFunction{J}{J}
    \SetKwFunction{fixed}{Fixed}
    \SetKwFunction{fix}{Fix}
    \SetKwFunction{neigh}{Neighbors}
    \SetKwFunction{neighsize}{NeighSize}
    \SetKwFunction{fixedneigh}{FixedNeigh}

	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
    \SetKwFor{ParFor}{for}{do in parallel}{endfor} 
    \DontPrintSemicolon
%     //same as in Algorithm~\ref{alg:distributed}
 	\Input{$\M,\varphi,{h}_{\mathit{max}},m,B, \beta, \cost$}
 	\Output{$\{\va^i\}_{1\leqslant i\leqslant\,m}$ \tcp*[l]{optimal control sequence}}
	\BlankLine
	Initialize $\ell_0\leftarrow J(s_0)$; $\widehat{J}\leftarrow\inf$;  $i\leftarrow 1$; $k\leftarrow B$;  $j\leftarrow 0$;
	\BlankLine
	\While{($\ell_{i-1} > \varphi)$ $\land$ $(i < m+h_\mathit{max})$}
	{
      $\va^i \leftarrow \NaN$ \tcp*{Initially no bird has a fixed solution}
      \While (\tcp*[f]{while not all birds have fixed solution}) {$\lnot \fixed(\va^i) $} {
        \tcp{Find $k$ nearest neighbors of $j$}
        $N_j \leftarrow \neigh(j, k)$\;
        \tcp{Get the states and the solutions of $j$'s neighbors}
        \tcp{$\Pi$ is a projection operator}
        $s_{N_j} \leftarrow \Pi_{N_j}(s(\M))$, $\va_{N_j}
        \leftarrow \Pi_{N_j}(\va^i)$\;
        $\Delta_j \leftarrow \min(J(s_{N_j})/(m-i),J(s_{N_j}))$\;
        $[\va_j, J_j] \leftarrow \localampc(\cost, s_{N_j}, \va_{N_j}, \Delta_j, h_{max}, \beta)$
        
        \tcp{Fix the solutions obtained by $j$ for all its neighbors}
        \ForAll{$ b \in \neigh(j, k)$}{$\va^i(b) \leftarrow \va_{j}(b)$ \tcp*[f]{$\va^i(b)$,$\va_{j}(b)$ is the solution for bird $b$ in $\va^i$,$\va_{j}$}} 
        \tcp{Find the birds without a fixed solution}
        $R \leftarrow \{j' \,|\, 1 \leqslant j' \leqslant B \land \lnot \fixed(\va^i_{j'})\}$\;
        \tcp{If all birds have fixed solution, the last bird that runs $\localampc$ becomes the first bird to run in the next time step. Otherwise we pick the bird that has the most neighbors with a fixed solution (if there are multiple such birds we pick the one with the smallest id).}
        \If{$R \neq \emptyset$}{
        $j \leftarrow \min \{j' \in R \,|\, \forall_{j'' \in R}\, \fixedneigh(j', k, \va^i) \geqslant \fixedneigh(j'', k, \va^i)\}$
        }
      }
%       //same as in Algorithm~\ref{alg:distributed}
       $J' \leftarrow J(s(\M))$\;
       $\M \leftarrow \M^{\va^i_1}$ \tcp*{Apply the actions (birds apply the actions in parallel)}
       $k \leftarrow \neighsize(J(s(\M)), J', k)$ \tcp*{Adjust the neighborhood size}
	}
	\caption{DAMPC}
	\label{alg:fixed_dampc}
\end{algorithm}
\setlength{\floatsep}{1cm}



==> ampc.tex <==
\section{Adaptive-Horizon Model Predictive Control}
\label{sec:ampc}

Our decentralized controller uses an
\emph{adaptive-horizon} MPC algorithm (\ampc).
The \ampc procedure is based on particle swarm optimization (\pso)~\cite{Kennedy95particleswarm} and used by a bird to obtain the optimal accelerations for its fixed neighborhood. 
%\ampc is an MPC procedure based on particle swarm optimization (\pso)~\cite{Kennedy95particleswarm}.

\ampc performs step-by-step control of a given MDP $\M$ by looking $h$ steps ahead---i.e.~it uses a \emph{prediction horizon} of length $h$---to determine the next optimal control action to apply. \pso is employed to solve the optimization problem generated by the MPC procedure. Since \pso is a randomized algorithm, \ampc is, in turn, a randomized controller.

For V-formation, the cost of a sequence $\va^h$ of $h$ accelerations is the minimum cost metric $J$ (Eq.~\ref{eq:cost}) obtained within $h$ steps by applying accelerations $\va^h$ on $\M$. Formally:
\begin{align}
\texttt{cost}(\M,\va^h,h) = \min_{1\leqslant \tau \leqslant h}{J(s_{\va^h}^\tau)}
\label{eq:ampcfit}
\end{align}
where $s_{\va^h}^\tau$ is the state of $\M$ obtained after applying the $\tau$-th action of $\va^h$ to the initial state of $\M$.\footnote{The initial state of $\M$ is being used to store the ``current'' state of the MDP as we execute our algorithm.} For horizon $h$, \pso searches for the best sequence of acceleration vectors of length $h$, thus having $2hB$ parameters to be optimized. The number of particles $p = 2\beta h B$ used in \pso is proportional to the number of parameters, and $\beta$ is a preset constant.

The \ampc procedure is given in Algorithm~\ref{alg:ampc}. Its main novelty is that, unlike classical MPC, which uses a fixed horizon $h$, it adaptively chooses $h$ depending on whether it is able to decrease the cost by a chosen quanta $\Delta_i$, $0 \leqslant i \leqslant m$, for $m$ steps. \ampc is, therefore, an adaptive MPC that uses level-based horizons. \ampc employs Matlab toolbox $\texttt{particleswarm}$, which performs the classical version of \pso. In contrast to the plan synthesis approach proposed in~\cite{lukina_tacas17}, Algorithm~\ref{alg:ampc} outputs the best control action at each step instead of a complete multi-segment plan sequence. It is designed to be deployed on-the-fly on a real plant. 

If actions $\va^h$ decrease $\texttt{cost}(\M,\va^h,h)$, the cost of the state reached within $h$ steps, by a predefined amount $\Delta_i$, then the controller considers these actions to be worthy of leading the flock towards, or keeping it in, a V-formation.\footnote{We focus on bird flocking, but our approach generalizes to other MDPs that come equipped with a cost metric.} In this case, the controller applies the first action to each bird and transitions to the next state of the MDP. The horizon $h$ is reset to $1$, the improvement $\Delta_i$ required in the next step is set, and other parameters are set (lines 6-10 of Algorithm~\ref{alg:ampc}).
% ASHISH: The following sentence is false, and hence commented out.
%Threshold $\Delta_i$ determines the next level $\ell_i\,{=}\,\texttt{cost}(\M,\widehat{\va}^h,h)$, where $\widehat{\va}^{h}$ is the optimal action sequence. 

If actions $\va^h$ do not decrease $\texttt{cost}(\M,\va^h,h)$, the cost of the state reached within $h$ steps, by the predefined $\Delta_i$, then the horizon $h$ is increased by one.  Also, the parameters for the underlying \pso are reset (line~12 of Algorithm~\ref{alg:ampc}).

If \ampc uses a horizon ${h}\,{>}\,1$, then the MDP needs to take multiple transitions to reach a state with sufficiently improved cost. However, when \ampc uses $h > 1$ to find such a state, we only apply the first action to transition the MDP to the next state, as in standard model-predictive control. In the next step, \ampc recomputes its optimal action for the actual state of the controlled plant in the next step.  Note that the actual next state of the flock may be quite different from the state predicted by \ampc, since birds outside ``my neighborhood'' might become part of ``my neighborhood'' in the next step.  This is a consequence of the decentralized nature of \dampc. 
%
If no new level is reached within a horizon of $h_{\mathit{max}}$, the first action of the best $\va^h$ using horizon $h_{\mathit{max}}$ is applied. 

The dynamic threshold $\Delta_i$ is defined as in~\cite{lukina_tacas17}: $\Delta_0$ equals the initial cost difference divided by $m$, that is, $\Delta_0\,{=}\,(\ell_0\,{-}\,\ell_m)\,{/}\,m$, where $\ell_0\,{=}\,J(s_0)$ and $\ell_m\,{=}\,\varphi$. Subsequently, $\Delta_i\,{=}\,\ell_{i-1}{/}(m\,{-}\,i\,{+}\,1)$ is determined by the previously reached level $\ell_{i-1}$. In this way, \ampc advances only if $\ell_i\,{=}\,\texttt{cost}(\M,\widehat{\va}^h,h)$ is at least $\Delta_i$ apart from $\ell_{i-1}$.
%$\ell_{i-1}\,{=}\,J(s_{k})$.

This adaptive-horizon approach allows us to force the \pso algorithm to escape from a local minimum, even if this implies passing over a cost bump, by gradually increasing the exploration horizon $h$.  The \ampc procedure can guarantee convergence if we make two assumptions. First, the MDP is controllable, i.e., it is possible to go from any state to any other state using an appropriate sequence of actions. Second, the set $G$ of good states is non-empty. Together the two assumptions imply that from any state, it is possible to reach a state whose cost is lower by at least $\Delta_i$. Algorithm~\ref{alg:ampc} provides the pseudocode for \ampc. %illustrates this approach.

\input{algo_ampc}

\begin{theorem}[AMPC]
%[\ampc Convergence]
\label{thm:ampc}
Given an MDP $\M\,{=}\,(S,A,T,J)$ with a positive and continuous cost function $J$, and a nonempty set of target states $G\,{\subset}\,S$ with $G\,{=}\,\{s\,|\,J(s)\,{\leqslant}\,\varphi\}$. If the transition relation $T$ is controllable with actions in $A$, and if PSO is assumed to return optimum solutions with high probability, then \ampc finds a sequence of actions $\va_1,\ldots,\va_m$ that brings a state in $S$ to a state in $G$ with probability that approaches $1$ as we increase the maximum horizon $h_\mathit{max}$ and the maximum number $m$ of execution steps.
%there exists a finite (maximum) horizon $h_{\mathit{max}}$ and a finite (maximum) number of execution steps $m$, such that \ampc is able to find a sequence of actions $\va_1,\ldots,\va_m$ that brings a state in $S$ to a state in $G$ with probability one.
\end{theorem}

\begin{proof}(Sketch)
If \ampc terminates in less-than $m$ steps, then it means it converged to a state in $G$. If not, then in the $m$-th step, and in every subsequent step, the desired reduction in cost, $\Delta_i$, equals the current cost $\ell_i$ (for $i \geq m$). So, in the $m$-th, $m+1$-st, $\ldots$i, $m+h_\mathit{max}$-th steps, \ampc will keep increasing the horizon $h$ until it finds a path to $G$. Since $\M$ is controllable, for some large $h$, such a path exists. Since PSO is assumed to not fail (to find best solutions) forever, this path will be found with probability that increases with $h_\mathit{max}$.
%In each (macro-)step of horizon length $h$, if $\ampc$ $h < h_{\mathit{max}}$, then \ampc goes from level $\ell_{i-1}$ to level $\ell_i$ and decreases the distance to $\varphi$ by $\Delta_i\,{\geqslant}\,\Delta$, where $\Delta\,{>}\,0$ is fixed by the number of steps $m$ chosen in advance. Hence, \ampc converges to a state in $G$ in finitely many steps. Now, \ampc will be able to decrease the cost in a macro-step by $\Delta_i$ with arbitrarily high probability if we increase $h_\mathit{max}$ because $\M$ is controllable, and by assuming that \pso is fair (finds a best solution). Since \pso and therefore \ampc are randomized algorithms, the result is probabilistic. 
\end{proof}

Note that Theorem~\ref{thm:ampc} is an existence theorem about $h_{\mathit{max}}$ and $m$. In practice, these values are chosen empirically. 
%Note also that \ampc is a significant contribution of our work. 
Traditional MPC uses a fixed horizon to determine the best control action, and can, therefore, get stuck in local minima. Hence, there is no global convergence guarantee for traditional MPC.  In contrast, \ampc dynamically chooses the horizon such that it reaches the next level. This, in turn, ensures convergence to a global minimum.
%which dynamically configures the amount of the effort it uses to search for a better solution at each step.  In~\cite{} the monolithic synthesis procedure was adaptive (and involved dynamically changing several parameters), whereas here the control procedure is adaptive and the underlying optimization is a non-adaptive off-the-shelf procedure, and hence the overall procedure here is simpler.
Finally, note that \ampc is a general procedure that performs adaptive MPC using \pso for any dynamical systems that are controllable, come with a cost metric, and have at least one optimal solution. %In an adversarial situation two players have opposing objectives. The question arises what one player assumes about the other when computing its own action, which we discuss next.
%\ampc is inspired by ARES~\cite{lukina_tacas17}. 

==> neighbors_graph_2.tex <==
% \definecolor{lavander}{cmyk}{0,0.48,0,0}
% \definecolor{violet}{cmyk}{0.79,0.88,0,0}
% \definecolor{burntorange}{cmyk}{0,0.52,1,0}

\def\lav{cyan!50}
\def\oran{yellow!50}

\tikzstyle{birds}=[draw,circle,black,fill=\lav,
                  text=black,minimum width=10pt]
\tikzstyle{fixedbirds}=[draw,rectangle,black,fill=black,
                  text=white,minimum width=10pt]
\tikzstyle{chosenbirds}=[draw,circle, black, fill=\oran,
                       text=black,minimum width=25pt]
\tikzstyle{legendcb}=[rectangle, draw, black, rounded corners,
                     thin,fill=\oran,
                     text=black, minimum width=2.5cm]
\tikzstyle{legendfb}=[rectangle, draw, black, rounded corners,
                     thin,fill=black,
                     text=white, minimum width=2.5cm]
\tikzstyle{legendb}=[rectangle, draw, black, rounded corners, thin,fill=\lav,
                     text= black, minimum width= 2.5cm]
\tikzstyle{legend_general}=[rectangle, rounded corners, thin,
                           black, fill= white, draw, text=black,
                           minimum width=2.5cm, minimum height=0.8cm]

\begin{tikzpicture}[auto, thick]
  \node[birds] (a1) at (-0.5,0.7) {$1$};
  \node[chosenbirds] (a2) at (-0.2,1.5) {$2$};
  \node[birds] (a3) at (0.4,2.1) {$3$};
  \node[birds] (a4) at (1,1.5) {$4$};
  \node[birds] (a6) at (1.9,0.5) {$6$};
  \node[birds] (a7) at (2.6,0) {$7$};
  \node[birds] (a5) at (1.8,1.4) {$5$};
  
  \path (a2) edge (a1);
  \path (a2) edge (a3);
  \path (a2) edge (a4);
  
  \draw (-0.9,-0.6) rectangle (3,2.5) {};
\end{tikzpicture}
\begin{tikzpicture}[auto, thick]
  \node[fixedbirds] (a1) at (-0.5,0.7) {$1$};
  \node[fixedbirds] (a2) at (-0.2,1.5) {$2$};
  \node[fixedbirds] (a3) at (0.4,2.1) {$3$};
  \node[fixedbirds] (a4) at (1,1.5) {$4$};
  \node[birds] (a6) at (1.9,0.5) {$6$};
  \node[birds] (a7) at (2.6,0) {$7$};
  \node[chosenbirds] (a5) at (1.8,1.4) {$5$};
  
  \path (a5) edge (a6);
  \path (a5.north) edge (a3);
  \path (a5) edge (a4);
  
  \draw (-0.8,-0.6) rectangle (3,2.5) {};
\end{tikzpicture}
\begin{tikzpicture}[auto, thick]
  \node[fixedbirds] (a1) at (-0.5,0.7) {$1$};
  \node[fixedbirds] (a2) at (-0.2,1.5) {$2$};
  \node[fixedbirds] (a3) at (0.4,2.1) {$3$};
  \node[fixedbirds] (a4) at (1,1.5) {$4$};
  \node[fixedbirds] (a6) at (1.9,0.5) {$6$};
  \node[chosenbirds] (a7) at (2.6,0) {$7$};
  \node[fixedbirds] (a5) at (1.8,1.4) {$5$};
  
  \path (a7.north) edge (a5);
  \path (a7.north) edge (a6);
  \path (a7.north) edge (a4);
  
  \draw (-0.8,-0.6) rectangle (3.1,2.5) {};
\end{tikzpicture}

==> related.tex <==
\section{Related Work}
\label{sec:related}
Prior work on the V-formation problem has focused on giving combinations of \emph{dynamical flight rules} as driving forces. These approaches tend to be distributed in nature, as flight rules describe how an individual bird maneuvers depending on the positions and velocities of the neighbors within its radius of influence.  

For instance, in~\cite{flake1998computational}, the authors extend Reynolds' flocking model~\cite{reynolds1987flocks} with a rule that forces a bird to move laterally away from any bird that blocks its view. This can result in multiple V-shaped clusters, but flock-wide convergence is not guaranteed. The work of~\cite{dimock2003aerodynamic} induces V-formations by extending Reynolds' model with a \emph{drag reduction} rule,
%% by which each bird reduces the power consumption via computing the
%% induced drag gradient and producing an acceleration along this
%% gradient. Their model produces flocks of Vs,
but the final formation tends to oscillate as birds repeatedly adjust the angle of the~V. Another approach, based on three \emph{positioning rules}, is that of~\cite{nathan2008}.
%% provides an alternative model that produces V-formations. The birds
%% in their model follow three positioning rules: (1) seek the proximity
%% of the nearest bird; (2) seek the nearest position that affords an
%% unobstructed longitudinal view; and (3) attempt to position itself in
%% the upwash of a leading bird.
Their model, however, is limited by the assumption that the birds have a constant longitudinal heading. The authors of~\cite{stonedahl2011finding} attempt to improve upon this approach by handling \emph{turning movements}. This also forms small clusters of birds, each of which is only moderately V-like.

In~\cite{lovethyneighbor16}, a classical MPC is used for V-formation control. The focus there is on a centralized control. We, in contrast, view the problem of V-formation as one of \emph{distributed optimal control}. Compared to previous work, there are no behavioral rules in our approach. Instead, we extend the technique of Adaptive-Horizon MPC~\cite{attackingV} to the distributed setting and successfully solve the V-formation problem. 
%the idea of model predictive control (MPC)~\cite{camacho2013model}.  To drive a collection of $N$ birds towards the desired formation, an optimal \emph{velocity adjustment} (acceleration) is performed at each time-step on each bird's current velocity using a model-based prediction window of $T$ time-steps.  This yields an optimal acceleration sequence of length $T$, and the first acceleration in the sequence is applied.
%We present both centralized and distributed versions of this approach.  
Moreover, in rule-based approaches, no attempt is made to dynamically reconfigure a bird's neighborhood size, which in the rule-based setting is determined by a fixed radius of influence. In contrast, we perform dynamic neighborhood resizing based on the current fitness (cost) of the flock. 

In~\cite{ZhanL13}, the problem of taking an arbitrary initial configuration of $n$ agents to a final configuration where every pair of ``neighbors'' is a fixed distance $d$ apart, and every agent is stationary (its velocity is zero) is considered. They present centralized and distributed algorithms for this problem, both of which use MPC to determine the next action. The problem addressed in~\cite{ZhanL13} is arguably simpler than the V-formation problem we consider. The cost function being minimized in their case is a quadratic convex function. In~\cite{ZhanL13} the proof of convergence uses the fact of existing sequence of states with monotonically decreasing cost. Our cost function is nonconvex and nonlinear, which requires overcoming local minima by horizon and neighborhood adaptation. Both of these concepts are not required, and hence not addressed, in~\cite{ZhanL13}. In the distributed control procedure of~\cite{ZhanL13}, each agent publishes the control value it locally computed, which is then used by other agents to compute their control value. A quadratic number of these ``small steps'' are performed before each agent fixes its control input for the next time step. Our distributed procedure has at most a linear number of these small steps.

Other related work, including~\cite{Fowler02,Dandrea03,Ye17}, focuses on distributed controllers for flight formation that operate in an environment where the (multi-agent) plant is already in the desired formation and the (distributed) controller's objective is to maintain formation in the presence of disturbances (typically on the roll angle of the wing). Moreover, the plants considered are more physically detailed than our plant model in terms of capturing the dynamics of moving-wing aircraft. We plan to consider models of this nature as future work. 

A distinguishing feature of these approaches is the particular formation they are seeking to maintain, including a half-vee~\cite{Fowler02}, a ring and a torus~\cite{Dandrea03}, and a leader-follower formation~\cite{Ye17}.  In contrast, we use distributed AMPC with dynamic neighborhood resizing to bring a flock from a mostly random initial configuration to a stable V-formation.

While our main focus here is on adaptive neighborhood resizing, for completeness, we mention previous work on adaptive-horizon MPC. In~\cite{droge2011adaptive}, AMPC
was used to track a reference signal, and a smaller horizon was applied in case of a poor estimate of the future behavior of the reference signal. We consider cost-based reachability goals here, which allows us to choose a horizon in a more generic way based on the progress toward the goal. More recently, adaptive horizons were also employed in~\cite{krener2016adaptive} for a reachability goal. However, they chose a large-enough horizon that enabled the system to reach states from where a pre-computed local controller could guarantee reachability of the goal. This is less practical than our approach for establishing the horizon.



==> subjidx.tex <==
%                                                           clmomu01.ind
%-----------------------------------------------------------------------
% CLMoMu01 1.0: LaTeX style files for books
% Sample index file for User's guide
% (c) Springer-Verlag HD
%-----------------------------------------------------------------------
\begin{theindex}
\item Absorption\idxquad 327
\item Absorption of radiation \idxquad 289--292,\, 299,\,300
\item Actinides \idxquad 244
\item Aharonov-Bohm effect\idxquad 142--146
\item Angular momentum\idxquad 101--112
\subitem algebraic treatment\idxquad 391--396
\item Angular momentum addition\idxquad 185--193
\item Angular momentum commutation relations\idxquad 101
\item Angular momentum quantization\idxquad 9--10,\,104--106
\item Angular momentum states\idxquad 107,\,321,\,391--396
\item Antiquark\idxquad 83
\item $\alpha$-rays\idxquad 101--103
\item Atomic theory\idxquad 8--10,\,219--249,\,327
\item Average value\newline ({\it see also\/} Expectation value)
15--16,\,25,\,34,\,37,\,357
\indexspace
\item Baker-Hausdorff formula\idxquad 23
\item Balmer formula\idxquad 8
\item Balmer series\idxquad 125
\item Baryon\idxquad 220,\,224
\item Basis\idxquad 98
\item Basis system\idxquad 164,\,376
\item Bell inequality\idxquad 379--381,\,382
\item Bessel functions\idxquad 201,\,313,\,337
\subitem spherical\idxquad 304--306,\, 309,\, 313--314,\,322
\item Bound state\idxquad 73--74,\,78--79,\,116--118,\,202,\, 267,\,
273,\,306,\,348,\,351
\item Boundary conditions\idxquad 59,\, 70
\item Bra\idxquad 159
\item Breit-Wigner formula\idxquad 80,\,84,\,332
\item Brillouin-Wigner perturbation theory\idxquad 203
\indexspace
\item Cathode rays\idxquad 8
\item Causality\idxquad 357--359
\item Center-of-mass frame\idxquad 232,\,274,\,338
\item Central potential\idxquad 113--135,\,303--314
\item Centrifugal potential\idxquad 115--116,\,323
\item Characteristic function\idxquad 33
\item Clebsch-Gordan coefficients\idxquad 191--193
\item Cold emission\idxquad 88
\item Combination principle, Ritz's\idxquad 124
\item Commutation relations\idxquad 27,\,44,\,353,\,391
\item Commutator\idxquad 21--22,\,27,\,44,\,344
\item Compatibility of measurements\idxquad 99
\item Complete orthonormal set\idxquad 31,\,40,\,160,\,360
\item Complete orthonormal system, {\it see}\newline
Complete orthonormal set
\item Complete set of observables, {\it see\/} Complete
set of operators
\indexspace
\item Eigenfunction\idxquad 34,\,46,\,344--346
\subitem radial\idxquad 321
\subsubitem calculation\idxquad 322--324
\item EPR argument\idxquad 377--378
\item Exchange term\idxquad 228,\,231,\,237,\,241,\,268,\,272
\indexspace
\item $f$-sum rule\idxquad 302
\item Fermi energy\idxquad 223
\indexspace
\item H$^+_2$ molecule\idxquad 26
\item Half-life\idxquad 65
\item Holzwarth energies\idxquad 68
\end{theindex}

